Reconstructing firm-level input-output networks from partial information

There is a large consensus on the fundamental role of firm-level supply chain networks in macroeconomics. However, data on supply chains at the fine-grained, firm level are scarce and frequently incomplete. For listed firms, some commercial datasets exist but only contain information about the existence of a trade relationship between two companies, not the value of the monetary transaction. We use a recently developed maximum entropy method to reconstruct the values of the transactions based on information about their existence and aggregate information disclosed by firms in financial statements. We test the method on the administrative dataset of Ecuador and reconstruct a commercial dataset (FactSet). We test the method's performance on the weights, the technical and allocation coefficients (microscale quantities), two measures of firms' systemic importance and GDP volatility. The method reconstructs the distribution of microscale quantities reasonably well but shows diverging results for the measures of firms' systemic importance. Due to the network structure of supply chains and the sampling process of firms and links, quantities relying on the number of customers firms have (out-degrees) are harder to reconstruct. We also reconstruct the input-output table of globally listed firms and merge it with a global input-output table at the sector level (the WIOD). Differences in accounting standards between national accounts and firms' financial statements significantly reduce the quality of the reconstruction.

==> figures/tikz_ntwk_example.tex <==
\begin{figure}[!htbp]
\centering
\begin{subfigure}{0.46\textwidth}
\begin{tikzpicture}[node distance =2 cm and 3cm ,
roundnode/.style={circle, draw=black, fill=white, minimum size=3mm},
]
% Nodes
\node[roundnode](A){$v_1$};
\node[roundnode](B)[left=of A]{$v_2$};
\node[roundnode](C)[below right=of A]{$v_3$};
\node[roundnode](D)[below left=of A]{$v_4$};
% Lines
\draw[line width=0.2mm, ->, >=latex] (A.west) --node [text width=0.5cm,midway,above,align=center]{4} (B.east);
\draw[line width=0.2mm, ->, >=latex] (A.south west) --node [text width=0.5cm,midway,left,align=center]{?} (D.north east);

\draw[line width=0.2mm, ->, >=latex] (B.south east) --node [auto]{?} (C.west);

\draw[line width=0.2mm, ->, >=latex] (C.north west) --node [text width=0.5cm,midway,above,align=center]{2} (A.south east);
\draw[line width=0.2mm, ->, >=latex] (C.south west) --node [text width=0.5cm,midway,below,align=center]{?} (D.east);

\draw[line width=0.2mm, ->, >=latex] (D.north west) --node [text width=0.5cm,midway,left,align=center]{?} (B.south);
\draw[line width=0.2mm, ->, >=latex] (D.east) --node [text width=0.5cm,midway,right,align=center]{?} (A.south);

\end{tikzpicture}
\end{subfigure}%
\begin{subfigure}{0.4\textwidth}
\begin{equation*}
\bm{W} =
\begin{blockarray}{ccccc}
&v_1 & v_2 & v_3 & v_4\\
\begin{block}{c[cccc]}
    v_1 & 0 & ? & 0 & 4 \\
    v_2 & 0 & 0 & ? & 0 \\
    v_3 & 2 & 0 & 0 & ?\\
    v_4 & ? & ? & 0 & 0 \\
\end{block}
\end{blockarray}
\end{equation*}

\end{subfigure}
\caption{Weighted directed network (on the left) and its adjacency matrix (on the right). Arrows indicate the direction of material flows}
\label{fig:WDgraph_example}
\end{figure}



==> tables/Nfirms_edges_avDeg_FactSet.tex <==
\begin{table}[!htbp]
\centering
\def\arraystretch{1.2}
\begin{tabular}{*{3}{c}}
\toprule
Number of nodes & Number of edges & Average degree\\
\midrule
5,442 & 15,916 & 2.9 \\
\bottomrule
\end{tabular}
\caption{Summary statistics for the 2014 FactSet network.}
\label{tab:Nfirm_overT_factset}
\end{table}


%\multicolumn{3}{l}{%
%\begin{minipage}{11cm}~\\%
%\justifying
%\noindent
%\footnotesize \textit{Notes}: The summary statistics are for the 2014 network for which we have cleaned financial statements and before introducing the proxy node.
%  \end{minipage}%
%}

==> tables/financials_variable_descr.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{p{0.18\textwidth}p{0.78\textwidth}}
\toprule
Variable & Description \\
\midrule
Revenues & Sales of goods and services earned from the company's core and recurring operations. \\

Cost of goods sold & The direct costs of production and/or services rendered incurred in the revenue generation process during the period. \\
 
Labour expenses & The total compensation to employees for services relating to the company's operations. It is disclosed in the income statement only if the company reports a by-nature income statement (Appendix~\ref{app:methods_income_statem} for the different methods to write the income statement), although companies using the by-function method might disclose labour expenses in a footnote. (For firms that have missing values, we estimate their labour expenses; see Appendix~\ref{app:constr_labor_exp}.)\\

Depreciation and amortisation & The total periodic allocation of the capitalised costs pertaining to property, plant and equipment, natural resources, intangible assets (including goodwill) and deferred charges to the income statement over the asset's useful life. \\

EBIT & A company's earnings before interests and taxes, i.e., its operating income. EBIT is calculated by subtracting the cost of goods sold, selling, general and administrative expenses, and other operating expenses from the revenues.\\

Value-added & Sum of labour expenses, EBIT, amortisation and depreciation (see Appendix~\ref{app:value_added} for more details). \\
\bottomrule
\end{tabular}
\caption{Description of the income statement variables used from the FactSet data set.}
\label{tab:vars_financials}
\end{table}

==> tables/summary_stas_ntwrks.tex <==
\begin{table}[!htbp]
\centering
\def\arraystretch{1.2}%  1 is the default
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c}
\toprule
Summary statistic & Scale-free & US 474 sectors & Ecuador \\
\midrule
N. nodes & 1,006 & 474 & 17,934 \\
N. edges & 2,973 & 25,301 & 2,165,002 \\
Network density & 0.003 & 0.11 & $6.7\times 10^{-3}$ \\
Average degree & 2.9 & 51.7 & 120.7 \\
N. weakly connected components & 1 & 1 & 1\\
N. strongly connected components & 1 & 36 & \\
Size weakly giant connected component & 1,006 (1.00) & 474 (1.00) & \\
Size strongly giant connected component & 1,006 (1.00) & 439 (0.93) & \\
\bottomrule
\end{tabular}
%}
\caption{Summary statistics for the scale-free network with 1,006 nodes, the US inter-industry transaction matrix with $N = 474$ and Ecuador's 2014 network composed of the firms in the weakly connected components of the network comprising the largest 20,000 firms (ranked by the out-strength). Numbers in parenthesis are normalized by $N$, the number of nodes.}
\label{tab:summary_stats_test_ntwks}
\end{table}




==> tables/table_variables_definition.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{p{0.2\textwidth}p{0.8\textwidth}}
\toprule
Notation & Description \\
\midrule
$q_i$ & firm $i$'s total sales \\
$q_s$ & sector $s$' gross output \\

$d_i$ & firm $i$'s intermediate sales \\
$d_s$ & sector $s$' intermediate sales \\

$x_i$ & firm $i$'s intermediate expenditure. We use the cost of goods sold cleaned from labour expenses. \\
$x_s$ & sector $s$' intermediate expenditure \\

$f_i$ & firm $i$'s final demand \\
$f_s$ & sector $s$' final demand. It comprises households and government demand but not NGOs final demand\\

$f_s^{np}$ & final demand of non-profit organisation for sector $s$. \\

$k_s$ & sector $s$' gross fixed capital formation \\

$\Delta n_s$ & changes in inventories and valuables of sector $s$\\

$w_i$ & firm $i$'s labour costs\\

$y_i$ & firm $i$'s value added. We use EBITDA plus labour costs. \\
$y_s$ & sector $s$' value added\\

$\tau$ & taxes minus subsidies on products of sector $s$\\

$e_s$ & CIF and FOB adjustments on exports of sector $s$\\
$p_s$ & direct purchases abroad by residents and purchases on the domestic territory by non-residents of sector $s$\\
$u_s$ & international transport margins of sector $s$\\

$Z_{r,s}$ & the amount of intermediate input sector $s$ buys from sector $r$\\

\bottomrule
\end{tabular}

\caption{Notation and terminology.}
\label{tab:vars_def}
\end{table}
